Unifying Bayesian Flow Networks and Diffusion Models through Stochastic Differential Equations

Bayesian flow networks (BFNs) iteratively refine the parameters, instead of the samples in diffusion models (DMs), of distributions at various noise levels through Bayesian inference. Owing to its differentiable nature, BFNs are promising in modeling both continuous and discrete data, while simultaneously maintaining fast sampling capabilities. This paper aims to understand and enhance BFNs by connecting them with DMs through stochastic differential equations (SDEs). We identify the linear SDEs corresponding to the noise-addition processes in BFNs, demonstrate that BFN's regression losses are aligned with denoise score matching, and validate the sampler in BFN as a first-order solver for the respective reverse-time SDE. Based on these findings and existing recipes of fast sampling in DMs, we propose specialized solvers for BFNs that markedly surpass the original BFN sampler in terms of sample quality with a limited number of function evaluations (e.g., 10) on both image and text datasets. Notably, our best sampler achieves an increase in speed of 5~20 times for free. Our code is available at https://github.com/ML-GSAI/BFN-Solver.

==> data/app-continuous-old.tex <==
\section{Derivation for Continuous-time BFN on Continuous Data}
\subsection{Proof of Theorem~\ref{thm:cbfn-sde}}
\label{proof:sde}
The proof is based on the Fokker–Planck–Kolmogorov equation. 
\begin{lemma}[Fokker–Planck–Kolmogorov equation]
The probability density of the solution of the SDE in Eq.~\eqref{eq:proof_sde} solves the partial differential equation(PDE):
    \begin{align}
        \frac{\partial p_t(\vmu)}{\partial t} = - &F(t)\sum_i \frac{\partial}{\partial \vmu_i} p_t(\vmu) + \frac{1}{2} G(t)^2 \sum_{i, j}\frac{\partial^2}{\partial \vmu_{i} \partial \vmu_{j}} {p_t(\vmu)}.
        \label{eq:FPK}
    \end{align}
\end{lemma}
\begin{proof}
According to the Theorem 5.2.1 in~\cite{oksendal2003stochastic}, the SDE in Eq.~\eqref{eq:proof_sde} has a unique solution if it satisfies the following regularity conditions:
\begin{enumerate}
    \item Condition 5.1.1~\cite{oksendal2003stochastic}: $\|F(t)\rvx\| + |G(t)| \leq C(1 + \|\rvx \|) \quad \forall \rvx \in \R^D, t \in [0,1]$ for some constant $C$.
    \item Condition 5.1.2~\cite{oksendal2003stochastic}: $\|F(t) \rvx - F(t) \rvy \| \leq D\| \rvx-\rvy\|  \quad \forall \rvx, \rvy \in \R^D, t \in [0,1]$ for some constant D.
\end{enumerate}
Note that $\lim_{t \rightarrow 1} f(t) \rightarrow \infty$ and Condition 5.1.1 is violated at $t=1$. Therefore, $t$ is truncated to fall within $[0, 1 - \eta]$.
% First, the SDE in~\eqref{eq:proof_sde} have a strong solution because the coefficients $f(t)\vmu$ and $g(t)$ satisfy  (Reason for  $\eta$).
% song: globally Lipschitz in both time and state 
Second, one could solve the partial differential equation in Eq.~\eqref{eq:FPK} to get density $p_t(\vmu)$. Alternatively, for the linear SDE in Eq.~\eqref{eq:proof_sde}, the solution is a linear transformation of Brownian motion, which is a Gaussian distribution whose mean and covariance have closed-form and can be obtained (see Sec. 5.5 in~\cite{Särkkä_Solin_2019}). With initial conditions $\vmu(0) \sim \mathcal{N}(\gamma(0)\rvx, \gamma(0)(1-\gamma(0)))$, the solution is
\begin{align}
     p(\vmu(t)) = \mathcal{N}(\vmu(t) | \vm_t, \mP_t),
\end{align}
where
\begin{align}
    \vm_t 
    =& e^{\int_0^t f(s) \dif s} \gamma(0)\rvx = \gamma(t) \rvx,\\
    \mP_t 
    =& \left(e^{2\int_0^t f(s) \dif s} \gamma(0)(1-\gamma(0)) + \int_0^t e^{2\int_\tau^t f(s)\dif s} g^2(\tau) d \tau \right)\mI = \gamma(t)(1-\gamma(t))\mI.
\end{align}
Therefore, the theorem holds because $p(\vmu(t)) = \mathcal{N}(\gamma(t) \rvx, \gamma(t)(1-\gamma(t))\mI)$ equals to $\flow(\vmu(t) | \rvx, \gamma(t))$ in Eq.~\ref{eq:bg-cbfn}. 
%Note that, in our SDE formulation, we use $\vmu_0$ as the final sample without an additional step to sample $\rvx$ from $\vmu_0$.
\end{proof}
\subsection{Proof of Proposition \ref{prop:convergence}}
\label{append:ancestral_sampling}
\begin{proof}
Given an initial value $\vmu(s)$ at time $s$, the exact solution at time $t$ of the reverse SDE in~\eqref{eq:cbfn-para-reverse-sde} is:
\begin{align}
    \vmu(t) = e^{\int_s^t f(\tau)d\dif \tau}\vmu(s) +  \int_s^t e^{\int_\tau^t f(r) \dif r} \frac{G(t)^2}{\sqrt{\gamma(t)(1-\gamma(t))}}\hat \epsilon(\vmu(\tau), \tau) \dif \tau + \int_s^t e^{\int_\tau^tf(r) \dif r} G(\tau) \dif \bar{\vw}_\tau.\label{eq:app_cts_sde_solu1}
\end{align}
Due to $\gamma(t)$ is a strictly decreasing function w.r.t $t$, we could rewrite Eq.~\eqref{eq:app_cts_sde_solu1} by change of variable $\gamma$ as:
\begin{align}
    \vmu(t) &= \frac{\gamma(t)}{\gamma(s)} \vmu(s) - 2\gamma(t)\int_{\gamma(s)}^{\gamma(t)} \frac{1}{\gamma\sqrt{\gamma(1-\gamma)}}\hat{\vepsilon}(\vmu({\gamma}), \gamma)\dif \gamma + \sqrt{\frac{\gamma(t)}{\gamma(s)}(\gamma(t)-\gamma(s))} \rvu_i\label{eq:app_cts_sde_solu2}.
\end{align}
where $\hat{\vepsilon}(\vmu(\gamma), \gamma) := \hat{\vepsilon}(\vmu(t_\gamma(\gamma)), t_\gamma(\gamma))$ and $t_\gamma(\cdot)$ is the inverse function fo $\gamma(t)$.
We could easily find that the sampling rule in~\eqref{eq:bg-cbfn-sample} can be written as a first-order discretization of the reverse SDE:
\begin{align}
    \vmu_{i} = & \frac{\gamma(t_i)}{\gamma_{t_{t-1}}} \vmu_{i-1} + \gamma(t_i)\int_{\gamma(t_{i-1})}^{\gamma(t_i)} \frac{1}{\gamma\sqrt{\gamma(1-\gamma)}}\hat{\vepsilon}(\vmu_{\gamma} ,\gamma)\dif \gamma + \sqrt{\frac{\gamma(t_i)}{\gamma(t_{i-1})}(\gamma(t_i)-\gamma(t_{i-1}))} \rvu_i \\
    = & \frac{\gamma(t_i)}{\gamma_{t_{t-1}}} \vmu_{i-1} +(\gamma(t_i) - \gamma(t_{i-1})) \frac{1}{\sqrt{\gamma(t_{i-1})(1 -\gamma(t_{i-1}))}} \hat{\vepsilon}(\vmu_{\gamma(t_{i-1})}, \gamma(t_{i-1})) + \sqrt{\frac{1-\gamma(t_i)}{1-\gamma(t_{i-1})}(\gamma(t_i) - \gamma(t_{i-1}))} \rvu_i \\
    & + O((\gamma(t_i) - \gamma(t_{i-1}))^2).
\end{align}
Comparing the sampling iteration rule of BFN in Eq.~\ref{eq:bg-cbfn-sample} and the exact solution of reverse-time SDE in Eq.~\ref{eq:app_cts_sde_solu2}. We find the sampler of BFN makes full use of the semi-linear property of reverse-time SDE which is different from the first-order Euler discretization. Note that in the implementation of BFN, the first two terms on the right of equaition~\eqref{eq:bg-cbfn-sample} are set to zero at the first step to avoid the numerical problem because $\gamma(t_0) = 0$. After sample $\vmu_n$, BFN sample from $\mathcal{N}(\rvx|\vmu_n, \sigma_1)$ to get final samples. 
\end{proof}
\subsection{Derivation of BFN-Solvers on Continuous Data}
\label{app:cts_bfn_solver}
Let time $t < s < 1-\eta$ and $\lambda(t) = \frac{1}{2}\log\frac{\gamma(t)}{1-\gamma(t)}$. The exact solution of the ODE in Eq.~\eqref{eq:cbfn-para-ode} can be formulated by "variation of constants" formula~\cite{atkinson2009numerical}:
\begin{align}
    \vmu(t) &= e^{\int_s^t f(\tau) \dif \tau} \vmu(s) + \int_s^t\left( e^{\int_\tau^t f(r)\dif r} \frac{g^2(\tau)}{ 2 \sqrt{\gamma(\tau)(1-\gamma(\tau))}}\hat{\vepsilon}(\mu_\tau, \tau) \right) \dif \tau.\label{eq:cts_exact_pro}
\end{align}
We can verify $\lambda(t)$ is a strictly decreasing function of $t$ by compute the derivative $\frac{\dif \lambda(t)}{\dif t} = -\frac{G(t)^2}{\gamma(t)(1-\gamma(t))} < 0$. Then we can rewrite Eq.~\eqref{eq:cts_exact_pro} as
\begin{align}
    \vmu(t) &= \frac{\gamma(t)}{\gamma(s)}\vmu(s) - \gamma(t) \int_{s}^{t} \frac{\dif \lambda(t)}{\dif \tau}\sqrt{\frac{1-\gamma(t)}{\gamma(t)}} \hat{\vepsilon}(\mu_{\tau}, \tau) \dif \tau\\
    &= \frac{\gamma(t)}{\gamma(s)}\vmu(s) - \gamma(t) \int_{\lambda(s)}^{\lambda(t)} e^{-\lambda} \hat{\vepsilon}(\vmu(t_\lambda(\lambda)), t_\lambda(\lambda)) \dif \lambda.
\end{align}
where $t_{\lambda}(\cdot)$ is the inverse function of $\lambda(t)$ as $\lambda(t)$ is a strictly decreasing function.
Given an initial value $\vmu_0$ and time steps $\{t_i\}_{i=0}^{n}$ from $t_0 = 1-\eta$ to $t_n = 0$. The solvers use $n$ steps to iteratively compute a sequence $\{\vmu_{i}\}_{i=1}^{n}$ to approximate the true solution at time $\{t_i\}_{i=1}^n$. Start with $\vmu_{i-1}$, according to Eq.~\ref{eq:cts_ode_exact}, the exact solution at $\vmu_{i}$ is 
\begin{align}
    \vmu_{i} \!=\! \frac{\gamma(t_{i})}{\gamma(t_{i-1})}\vmu_{i-1} \!-\! \gamma(t_{i}) \int_{\lambda(t_{i-1})}^{\lambda(t_{i})} e^{-\lambda} \hat{\vepsilon}(\mu(t_\lambda(\lambda)), t_\lambda(\lambda)) \dif \lambda.\label{eq:stc_ode_solver_integral}
\end{align}
Denote $\vepsilon^{(m)}(\mu(t_\lambda(\lambda)), t_\lambda(\lambda))  := \frac{\dif^m \hat{\vepsilon}(\mu(t_\lambda(\lambda)), t_\lambda(\lambda))}{\dif \lambda^m}$ as the $m$-th order total derivative of $\hat{\vepsilon}(\mu(t_\lambda(\lambda)), t_\lambda(\lambda))$, w.r.t. $\lambda$. For $k \geq 1$, the $(K-1)$-th order Taylor expansion of $\hat{\vepsilon}(\mu(t_\lambda(\lambda)), t_\lambda(\lambda))$ w.r.t. $\lambda$ at $\lambda(t_{i-1})$ is 
\begin{align}
    \hat{\vepsilon}(\mu(t_\lambda), t_\lambda)  =\sum_{m=0}^{k-1} \frac{\lambda - \lambda(t_{i-1})}{m!}\hat\vepsilon^{(m)}(\vmu(t_\lambda(\lambda)), t_\lambda(\lambda)) + \mathcal{O}(h_i^{k})
\end{align}
Substituting the above Taylor expansion into Eq.\eqref{eq:stc_ode_solver_integral} yields 
\begin{align}
    \vmu_{i} \!=\! \frac{\gamma(t_{i})}{\gamma(t_{i-1})}\vmu_{i-1} \!-\! \gamma(t_{i}) \sum_{m=0}^{k-1} \vepsilon^{(m)}(\vmu(t_\lambda(\lambda)), t_\lambda(\lambda))\int_{\lambda(t_{i-1})}^{\lambda(t_{i})} e^{-\lambda} \frac{\lambda - \lambda(t_{i-1})}{m!} \dif \lambda + \mathcal{O}(h_i^{k+1}).
\end{align}
where $\int_{\lambda(t_{i-1})}^{\lambda(t_{i})} e^{-\lambda} \frac{\lambda - \lambda(t_{i-1})}{m!} \dif \lambda$ can be analytically computed. By approximating the first $(k-1)$-th total derivate, we can derive $k$-th order solver for our ODE. A more straightforward way to get BFN-Solver on continuous data is to treat BFN as a DM with a special noise schedule $\alpha_t = \gamma_t$ and $\sigma^2_t = \gamma_t(1 - \gamma_t)$. Our implementation of first-order ODE solver named BFN-Solver1, second-order ODE solver named BFN-Solver2, first-order SDE solver named BFN-SDE-Solver1 and second-order SDE solver named BFN-SDE-Solver2 is are presented in Algorithm~\ref{ag:BFN-Solver-1-cts},~\ref{ag:BFN-Solver-2-cts},~\ref{ag:BFN-SDE-Solver-1-cts} and~\ref{ag:BFN-SDE-Solver-2-cts} respectively. 
\begin{algorithm}[tb]
   \caption{BFN-Solver-1(on continuous data)}
   \label{ag:BFN-Solver-1-cts}
\begin{algorithmic}
   \STATE {\bfseries Require:} time steps $\{t_i\}_{i=0}^{n}$ from $t_0 = 1- \eta$ to $t_n = 0$, noise prediction model $\hat{\vepsilon}$
   \STATE Denote $\bar{\alpha}_{t} = \gamma(t)$, $\bar{\sigma}_{t}= \sqrt{\gamma(t)(1-\gamma(t))}$, $\lambda_t = \log \frac{\bar \alpha_t}{\bar{\sigma}_t}$
   \STATE ${\vmu}_0 \sim \mathcal{N}(\textbf{0}, \gamma(t_0)(1-\gamma(t_0))\mI), K\beta(t_0)\mI)$
   \FOR{$i=1$ {\bfseries to} $n-1$}
   \STATE $h_i = (\lambda_{t_i} - \lambda_{t_{i-1}})$
   \STATE $\hat{\rvx}_i = \frac{\vmu_{i-1}}{\gamma(t_{i-1})} - \sqrt{\frac{1-\gamma(t_{i-1})}{\gamma(t_{i-1})}} \hat{\vepsilon}(\vmu_{i-1})$
   \STATE ${\vmu}_i = \frac{\bar{\sigma}_{t_i}}{\bar{\sigma}_{t_{i-1}}}{\vmu}_{i-1} - \bar{\alpha}_{t_i}(e^{-h_i} - 1) \hat{\rvx}_i$
   \ENDFOR
   \STATE $\hat{\rvx}_n = \frac{\vmu_{n-1}}{\gamma_{t_{n-1}}} - \sqrt{\frac{1-\gamma_{t_{n-1}}}{\gamma_{t_{n-1}}}} \hat{\vepsilon}(\vmu_{n-1})$
   \STATE {\bfseries return} $\hat {\rvx}_n$
\end{algorithmic}
\end{algorithm}
\begin{algorithm}[tb]
   \caption{BFN-Slover2(on continuous data)}
   \label{ag:BFN-Solver-2-cts}
\begin{algorithmic}
   \STATE {\bfseries Require:} time steps $\{t_i\}_{i=0}^{n}$ from $t_0 = 1- \eta$ to $t_n = 0$, noise prediction model $\hat{\vepsilon}$
   \STATE Denote $\bar{\alpha}_{t} = \gamma(t)$, $\bar{\sigma}_{t}= \sqrt{\gamma(t)(1-\gamma(t))}$, $\lambda_t = \log \frac{\bar \bar{\alpha}_t}{\bar{\sigma}_t}$
   \STATE ${\vmu}_0 \sim \mathcal{N}(\textbf{0}, \gamma(t_0)(1-
   \gamma(t_0))\mI), K\beta(t_0)\mI)$, Initialize an empty buffer $Q$.
   \STATE $\hat{\rvx}_{0} = \frac{\vmu_{0}}{\gamma_{t_{0}}} - \sqrt{\frac{1-\gamma_{t_0}}{\gamma_{t_0}}} \hat{\vepsilon}(\vmu_{0})$
   \STATE $Q \leftarrow \hat{\rvx}_{0}$
   \STATE $\vmu_{1} = \frac{\bar{\sigma}_{t_1}}{\bar{\sigma}_{t_0}}\vmu_{0} - \bar{\alpha}_{t_1}(e^{-h_1}-1) \hat{\rvx}_{0}$
    \STATE $\hat{\rvx}_{1} = \frac{\vmu_{1}}{\gamma_{t_{1}}} - \sqrt{\frac{1-\gamma_{t_1}}{\gamma_{t_1}}} \hat{\vepsilon}(\vmu_{1})$
   \STATE $Q \leftarrow \hat{\rvx}_{1}$
   \FOR{$i=2$ {\bfseries to} $n$}
   \STATE $h_i = (\lambda_{t_i} - \lambda_{t_{i-1}})$
   \STATE $r_i = \frac{h_{i-1}}{h_i}$
   \STATE $\mD_i = \left(1+ \frac{1}{2r_i}\hat{\rvx}_{t_{i-1}} - \frac{1}{2r_i}\hat{\rvx}_{i-2}\right)$
   \STATE ${\vmu}_i = \frac{\bar{\sigma}_{t_i}}{\bar{\sigma}_{t_{i-1}}} - \bar{\alpha}_{t_i}(e^{-h_i} - 1)\mD_i$
   \STATE $\hat{\rvx}_{i} = \frac{\vmu_{i}}{\gamma_{t_{i}}} - \sqrt{\frac{1-\gamma(t_i)}{\gamma(t_i)}} \hat{\vepsilon}(\vmu_{i})$
   \STATE If $i<n$, then $Q \leftarrow \hat{\rvx}_{i}$
   \ENDFOR
   \STATE {\bfseries return} $\hat{\rvx}_n$
\end{algorithmic}
\end{algorithm}
\begin{algorithm}[tb]
   \caption{BFN-SDE-Slover1(on continuous data)}
   \label{ag:BFN-SDE-Solver-1-cts}
\begin{algorithmic}
   \STATE {\bfseries Require:} time steps $\{t_i\}_{i=0}^{M}$ from $t_0 = 1- \eta$ to $t_M = 0$, noise prediction model $\hat{\vepsilon}$
   \STATE Denote $\bar{\alpha}_{t} = \gamma(t)$, $\bar{\sigma}_{t}= \sqrt{\gamma(t)(1-\gamma(t))}$, $\lambda_t = \log \frac{\bar \alpha_t}{\bar{\sigma}_t}$
   \STATE ${\vmu}_0 \sim \mathcal{N}(\textbf{0}, \gamma(t_0)(1-
   \gamma(t_0))\mI), K\beta(t_0)\mI)$, Initialize an empty buffer $Q$.
   \STATE $\hat{\rvx}_{0} = \frac{\vmu_{0}}{\gamma_{t_{0}}} - \sqrt{\frac{1-\gamma_{t_0}}{\gamma_{t_0}}} \hat{\vepsilon}(\vmu_{0})$
   \STATE $Q \leftarrow \hat{\rvx}_{0}$
   \STATE $\vmu_{1} = \frac{\bar{\sigma}_{t_1}}{\bar{\sigma}_{t_0}}\vmu_{0} - \bar{\alpha}_{t_1}(e^{-h_1}-1) \hat{\rvx}_{0}$
    \STATE $\hat{\rvx}_{1} = \frac{\vmu_{1}}{\gamma_{t_{1}}} - \sqrt{\frac{1-\gamma_{t_1}}{\gamma_{t_1}}} \hat{\vepsilon}(\vmu_{1})$
   \STATE $Q \leftarrow \hat{\rvx}_{1}$
   \FOR{$i=2$ {\bfseries to} $M$}
   \STATE $h_i = (\lambda_{t_i} - \lambda_{t_{i-1}})$
   \STATE $r_1 = \frac{h_{i-1}}{h_i}$
   \STATE $\mD_i = \frac{1}{r_1}(\hat{\rvx}_{i-1} - \hat{\rvx}_{i-2})$
   \STATE $\rvz_{t_{i-1}} \sim \mathcal{N}(\boldsymbol{0}, \mI)$
   \STATE ${\vmu}_i = \frac{\bar{\sigma}_{t_i}}{\bar{\sigma}_{t_{i-1}}}e^{-h_i}\vmu_{i-1} + \bar{\alpha}_{t_i}(1-e^{-2h_i} )\hat{\rvx}_{i-1} + \frac{\bar{\alpha}_t(1-e^{-2h_i})}{2}\mD_i + \bar{\sigma}_t \sqrt{1-e^{-2h_i}} \rvz_{t_{i-1}}$
   \STATE $\hat{\rvx}_{i} = \frac{\vmu_{i}}{\gamma_{t_{i}}} - \sqrt{\frac{1-\gamma(t_i)}{\gamma(t_i)}} \hat{\vepsilon}(\vmu_{i})$
   \STATE If $i<n$, then $Q \leftarrow \hat{\rvx}_{i}$
   \ENDFOR
   \STATE {\bfseries return} $\hat{\rvx}_M$
\end{algorithmic}
\end{algorithm}
\begin{algorithm}[tb]
   \caption{BFN-SDE-Slover2(on continuous data)}
   \label{ag:BFN-SDE-Solver-2-cts}
\begin{algorithmic}
   \STATE {\bfseries Require:} time steps $\{t_i\}_{i=0}^{M}$ from $t_0 = 1- \eta$ to $t_M = 0$, noise prediction model $\hat{\vepsilon}$
   \STATE Denote $\bar{\alpha}_{t} = \gamma(t)$, $\bar{\sigma}_{t}= \sqrt{\gamma(t)(1-\gamma(t))}$, $\lambda_t = \log \frac{\bar \alpha_t}{\bar{\sigma}_t}$
   \STATE ${\vmu}_0 \sim \mathcal{N}(\textbf{0}, \gamma(t_0)(1-
   \gamma(t_0))\mI), K\beta(t_0)\mI)$, Initialize an empty buffer $Q$.
   \STATE $\hat{\rvx}_{0} = \frac{\vmu_{0}}{\gamma_{t_{0}}} - \sqrt{\frac{1-\gamma_{t_0}}{\gamma_{t_0}}} \hat{\vepsilon}(\vmu_{0})$
   \STATE $Q \leftarrow \hat{\rvx}_{0}$
   \STATE $\vmu_{1} = \frac{\bar{\sigma}_{t_1}}{\bar{\sigma}_{t_0}}\vmu_{0} - \bar{\alpha}_{t_1}(e^{-h_1}-1) \hat{\rvx}_{0}$
    \STATE $\hat{\rvx}_{1} = \frac{\vmu_{1}}{\gamma_{t_{1}}} - \sqrt{\frac{1-\gamma_{t_1}}{\gamma_{t_1}}} \hat{\vepsilon}(\vmu_{1})$
   \STATE $Q \leftarrow \hat{\rvx}_{1}$
   \FOR{$i=2$ {\bfseries to} $M$}
   \STATE $h_i = (\lambda_{t_i} - \lambda_{t_{i-1}})$
   \STATE $r_1 = \frac{h_{i-1}}{h_i}$
   \STATE $\mD_i = \frac{1}{r_1}(\hat{\rvx}_{i-1} - \hat{\rvx}_{i-2})$
   \STATE $\rvz_{t_{i-1}} \sim \mathcal{N}(\boldsymbol{0}, \mI)$
   \STATE ${\vmu}_i = \frac{\bar{\sigma}_{t_i}}{\bar{\sigma}_{t_{i-1}}}e^{-h_i}\vmu_{i-1} + \bar{\alpha}_{t_i}(1-e^{-2h_i} )\hat{\rvx}_{i-1} + \frac{\bar{\alpha}_t(1-e^{-2h_i})}{2}\mD_i + \bar{\sigma}_t \sqrt{1-e^{-2h_i}} \rvz_{t_{i-1}}$
   \STATE $\hat{\rvx}_{i} = \frac{\vmu_{i}}{\gamma_{t_{i}}} - \sqrt{\frac{1-\gamma(t_i)}{\gamma(t_i)}} \hat{\vepsilon}(\vmu_{i})$
   \STATE If $i<M$, then $Q \leftarrow \hat{\rvx}_{i}$
   \ENDFOR
   \STATE {\bfseries return} $\hat{\rvx}_M$
\end{algorithmic}
\end{algorithm}

